SeeMoRe: A Fault-Tolerant Protocol for Hybrid Cloud Environments

Large scale data management systems utilize State Machine Replication to provide fault tolerance and to enhance performance. Fault-tolerant protocols are extensively used in the distributed database infrastructure of large enterprises such as Google, Amazon, and Facebook, as well as permissioned blockchain systems like IBM's Hyperledger Fabric. However, and in spite of years of intensive research, existing fault-tolerant protocols do not adequately address all the characteristics of distributed system applications. In particular, hybrid cloud environments consisting of private and public clouds are widely used by enterprises. However, fault-tolerant protocols have not been adapted for such environments. In this paper, we introduce SeeMoRe, a hybrid State Machine Replication protocol to handle both crash and malicious failures in a public/private cloud environment. SeeMoRe considers a private cloud consisting of nonmalicious nodes (either correct or crash) and a public cloud with both Byzantine faulty and correct nodes. SeeMoRe has three different modes which can be used depending on the private cloud load and the communication latency between the public and the private cloud. We also introduce a dynamic mode switching technique to transition from one mode to another. Furthermore, we evaluate SeeMoRe using a series of benchmarks. The experiments reveal that SeeMoRe's performance is close to the state of the art crash fault-tolerant protocols while tolerating malicious failures.

==> sec_alg_old.tex <==
\section{\protocol}\label{sec:alg}

In this section we present \protocol,
a hybrid fault-tolerant consensus protocol
for a public/private cloud environment
that tolerates $m$ malicious failures in the public
and $c$ crash failures in the private cloud.


\protocol in inspired by the known Byzantine fault-tolerant protocol PBFT \cite{kapitza2012cheapbft}.
In PBFT, as can be seen in Figure~\ref{fig:pbft},
during a normal case execution a client sends a request to a (primary) replica, and
the primary multicasts a {\tt "pre-prepare"} message to all replicas.
Then, during the {\tt "prepare"} and {\tt "commit"} phases, $3f+1$ replicas communicate
to reach an agreement and send responses back to the client.
Finally, the client waits for $f+1$ valid matching responses from different replicas
to make sure at least one correct replica executed its request.
PBFT also has a veiw change routine that provides liveness by allowing
the system to make progress when the primary fails.

\protocol consists of agreement and view change routines where
the agreement routine orders requests for execution by the replicas, and 
the view change routine coordinates the election of a new primary when
the current primary is faulty.

The algorithm, similar to most fault-tolerant algorithms,
is a form of state machine replication \cite{schneider1990implementing}.
In such approaches, a service is replicated across a group of servers
in a distributed system.
Each server maintains a set of state variables, which are
modified by a set of "atomic" and "deterministic" operations.
Operations are {\em atomic} if they do not interfere with each other and
{\em deterministic} if the same operation executed in the same initial state
generates the same final state.
Also, the initial state must be the same in all replicas. 


The algorithm has to satisfy two main properties,
(1) {\em safety}: all correct servers execute the same requests in the same order, and
(2) {\em liveness}: all correct client requests are eventually executed.
Fischer et al. \cite{fischer1985impossibility} show that 
in an asynchronous system, where nodes can fail,
consensus has no solution that is both safe and live.
Based on that impossibility result, most fault-tolerant protocols
satisfy the safety property without any synchrony assumption and
consider a synchrony assumption to satisfy the liveness property.
% Indeed, as long as the number of faulty nodes does not exceed the defined threshold,
% a protocol can produce linearizable executions,
% independent of whether the network loses, reorders, or arbitrarily delays messages.
% However, a weak synchrony assumption is needed to satisfy liveness:
% the delay from the moment when a request is sent by a client
% for the first time and the moment when it is received by its
% destination is in some fixed (but potentially unknown) interval.

We identify each replica using an integer in $[0,..., N{-}1]$ where
replicas in the private cloud, i.e., trusted replicas,
have identifiers in $[0, ..., S{-}1]$ and
replicas in the public cloud, i.e., untrusted replicas,
are identified using integers in $[S, ..., N{-}1]$.

In \protocol replicas move through a succession of configurations
called {\em views} \cite{el1985efficient}\cite{el1985availability}.
In a view, one replica is {\em the primary} and the others are {\em backups}.
Depending on the mode, some backups are {\em passive} and do not participate
in the agreement. Views are numbered consecutively.
All replicas are initially in view $0$ and
are aware of their current view number at all time.

We explain \protocol in three different modes:
{\em Lion}, {\em Dog}, and {\em Peacock}
\footnote{We call the modes Lion, Dog, and Peacock because seemorq (=SeeMoRe) is composed of these three animals.}
modes.
In the Lion mode, we assume that the primary is always in the private cloud,
thus the primary is non-malicious.
The Dog mode is used to reduce the load on the private cloud
by assuming that the primary is still in the private cloud, but
instead of processing the client requests itself,
depends on $3m+1$ nodes in the public cloud to process the request.
This mode 
reduces the load on the private cloud, because except for the the primary,
which does a single broadcast of the client's request,
other replicas in the private cloud are passive and do not participate in any phases.
Finally, in the Peacock mode, an untrusted node is allowed to be the primary and
the protocol relies completely on the public cloud to process requests.
This mode is helpful when
%either all trusted replicas may fail, i.e., $S=c$, or
we intentionally rely completely on the public cloud for two purposes:
(1) load balancing when all the nodes in the private cloud are heavily loaded, or
(2) reducing the delay when there is a large network distance between the private and the public cloud and
the latency of having one more phase is less than the latency of exchanging messages between the two clouds.
The agreement routine of the Peacock mode is the same as PBFT \cite{kapitza2012cheapbft},
However, the view change routine can be more efficient.


In this section, we describe each of these three modes in details.
For each mode,
we first present the normal-case operation of the protocol and
then show how view changes are carried out
when it appears that the primary has failed.
Next, we show how \protocol can
dynamically switch between these three modes.
We use $\pi$ to show the current mode of the protocol where $\pi \in \{1,2,3\}$.
At the end of this section, we also present a short discussion on different modes of \protocol and compare it
with some of the known relevant protocols, i.e.,
Paxos \cite{lamport2001paxos}, PBFT \cite{kapitza2012cheapbft}, and UpRight \cite{clement2009upright}.

  \begin{figure*}[t]
  \centering
  \subfigure[Lion Mode]{
  \label{fig:case1}
  \includegraphics[width=0.22\linewidth]{Lion.jpg}}
 % \quad
  \subfigure[Dog Mode]{
  \label{fig:case2}
  \includegraphics[width=0.22\linewidth]{Dog.jpg}}
  %\quad
  \subfigure[Peacock Mode]{
  \label{fig:case3}
  \includegraphics[width=0.25\linewidth]{Peacock.jpg}}
  %\quad
  \subfigure[PBFT]{
  \label{fig:pbft}
  \includegraphics[width=0.23\linewidth]{PBFT.jpg}}
  \caption{The normal case operation of the three modes of \protocol and PBFT}
  \label{fig:normalcase}
  \end{figure*}

\subsection{The Lion Mode: Trusted Primary} \label{sec:mode1}

\begin{algorithm}
\label{algo:lion}
\caption{Steps followed by the primary or a replica in {Lion mode}.}
\begin{algorithmic}[1]
\State \textbf{init():} 
\State    \quad $r$ := $replica\_ id$
\State    \quad $v$ := $view\_ number$ 
\State    \quad if $r = (v$ mod $S)$, $S$ is private network size:
\State        \qquad $is\_primary$ := \textsf{true\\}

\State \textbf{upon receiving} $\mu = \big\langle\REQ, op, ts_{\varsigma}, \varsigma \big\rangle_{\sigma_{\varsigma}}$ from client $\varsigma$ and \textbf{\textit{is\_primary = true}:}

\State    \quad if \textit{check\_valid\_req($\mu$):}
    
\State    \qquad $n$ := $sequence\_num$
    
\State    \qquad \textbf{send} $\big\langle\big\langle\text{\ONE}, v, n \big\rangle_{\sigma_p}, \mu \big\rangle$ to all {replicas\\}

\State \textbf{upon receiving} $\big\langle\big\langle\text{\ONE}, v, n \big\rangle_{\sigma_p}, \mu \big\rangle$ from primary:

\State    \quad if $v$ is valid:
    
\State    \qquad log the message
    
\State    \qquad \textbf{send} $\big\langle\text{\TWO}, v, n, r \big\rangle$ to {primary\\}

\State \textbf{upon receiving} $\big\langle\text{\TWO}, v, n, r \big\rangle$ from \textbf{2m + c} replicas and \textbf{\textit{is\_primary = true}}:

\State    \quad \textbf{send} $\big\langle \big\langle\text{\THREE}, v, n \big\rangle_{\sigma_p}, \mu \big\rangle$ to all replicas
    
\State    \quad \textbf{send} $\big\langle\text{\REPLY}, \pi, v, ts_{\varsigma}, u  \big\rangle_{\sigma_p}$ to client $\varsigma$ with mode number  $\pi$ and result $u$

\end{algorithmic}
\end{algorithm}
Owning a private cloud gives \protocol the chance to choose a trusted node
as the primary.
When the primary is trusted, all the non-faulty backups receive correct
messages from the primary, which
eliminates the need to multicast messages by replicas to
realize whether all the non-faulty ones receive the same message or not.
Thus, we can reduce one phase of communication and
a large number of messages.
In the first mode, the primary of view $v$ is a replica $p$ such that
$p = (v \mod S)$.

In particular, within a view, the normal case operation for \protocol
to execute a client request proceeds as follows.
A client sends a {\em \req} message to the primary,
i.e., a trusted replica in the private cloud.
The primary assigns a sequence number to the request and
multicasts a {\em \one} message including the request to all replicas.
Replicas receive a {\em \one} from the primary and send an {\em \two} to the primary.
The primary upon receiving $2m +c+1$ matching {\em \two} messages, sends a {\em \three} message to all replicas and a {\em \reply} to the client.
%Note that the replicas do not need to multicast their {\em \two} message since the primary can use the {\em \two} message from the trusted backup to filter malicious {\em \two} messages.
Upon receiving a {\em \three} message from the primary,
replicas execute the client request. Finally, the client receives a {\em \reply} message from the primary and marks the request as complete.

Figure~\ref{fig:case1} show the normal case operation of \protocol
in the Lion mode.
Here, replicas $0$ and $1$ are trusted ($S=2$) and
the four other replicas ($2$, $3$, $4$, and $5$) are untrusted ($P=4$).
In addition, one of the trusted replicas $(1)$ is crashed ($c=1$) and
one of the untrusted replicas $(5)$ is malicious ($m=1$).
As can be seen in Figure~\ref{fig:case1}, when the primary is trusted
the total number of exchanged messages is $3N$.

In the Lion mode of the protocol, view changes are carried out when it appears that the primary has failed.
When a set of backups suspect that the primary has crashed,
a view change operation is executed, and a new replica becomes the primary.
This mechanism provides liveness
by allowing the system to make progress when the primary is faulty.

The detailed explanation of the steps taken by \protocol to execute a
client request are as follows:

\medskip
\noindent
{\bf Step 1:}
A client $\varsigma$ requests a state machine operation $op$
by sending a message $\big\langle\REQ, op, ts_{\varsigma}, \varsigma \big\rangle_{\sigma_{\varsigma}}$
to the replica $p$ it believes to be the primary.
Here, $ts_\varsigma$ is  the client's timestamp and the entire message
is signed with signature $\sigma_{\varsigma}$.
We use timestamps of clients to totally order the requests of each client and to ensure exactly-once semantics for the execution of client requests.

\medskip
\noindent
{\bf Step 2:}
Each replica keeps the state of the service,
a message log containing valid messages the replica has received, and
an integer denoting the replica's current view number.
message logs then serve as the basis for maintaining consistency in view changes.

Upon receiving a \req message from a client,
primary $p$ first checks the signature and the timestamp.
Requests with an invalid signature $\sigma_{\varsigma}$ are simply discarded.
%Timestamp $ts$ is the request identifier that is used to ensure exactly-once semantics.
The primary also checks the timestamp of the last request that is executed
for client $\varsigma$ in its message log.
If the timestamp of the current request is less than the last executed request,
the request is discarded by the primary.

If both the signature and timestamp are valid,
the primary starts a {\em two-phase} protocol by assigning a sequence number, $n$,
to the request, forming a \one message along with the client request and multicasting
$\big\langle\big\langle\text{\ONE}, v, n \big\rangle_{\sigma_p}, \mu \big\rangle$
to all replicas
where $v$ is the view in which the message is being sent, and
$\mu$ is the client's request message.
At the same time, the primary appends the message to its log.
The primary signs its message, because it might be used by other replicas
later in view changes as a proof of receiving the message.

\medskip
\noindent
{\bf Step 3:}
Upon receipt of $\big\langle\big\langle\text{\ONE}, v, n, \big\rangle_{\sigma_p}, \mu \big\rangle$
from primary $p$,
if view $v$ is equal to the replica's view,
replica $r$ logs the \one message, and
forms a
$\big\langle\text{\TWO}, v, n, r \big\rangle$ message.
The replica sends the message to the primary and adds the message to its log.
Since \two messages are only sent to the trusted primary from the
communication channels and are not used later for any other purposes,
there is no need to sign these messages.

\medskip
\noindent
{\bf Step 4:}
When the primary receives an \two message,
if the view number is equal to its current view, the primary logs the message.
Upon collecting $2m+c$ valid \two messages from different replicas
(plus itself becomes $2m+c+1$)
for the request $\mu$ in view $v$ with sequence number $n$,
the primary forms a \three message
$\big\langle \big\langle\text{\THREE}, v, n \big\rangle_{\sigma_p}, \mu \big\rangle$
and multicasts to other replicas.
The primary attaches the request $\mu$ to its \three message,
so that if a replica has not received a \one message for that request,
it can still execute the request.
The primary also executes the request and sends a \reply message
$\big\langle\text{\REPLY}, \pi, v, ts_{\varsigma}, u  \big\rangle_{\sigma_p}$
to client $\varsigma$ where
$ts_{\varsigma}$ is the timestamp of the corresponding request,
$u$ is the result of executing the request,
$\pi$ is the mode, and $v$ is the view number.
Both \three and \reply messages are logged.

Mode number $\pi$ and view number $v$ are sent to clients to 
enable them to track the current mode and view and hence the current primary.
It is important especially when a mode change or view change happens and
the current primary is different from the primary of the view that client sent
its request.

Note that before sending the \three messages for request $\mu$,
the primary has to wait for $2m+c$ \two messages from different replicas
to ensure that committed requests are totally ordered across views.
This ensures that in the event of the failure of the primary,
any new quorum of $2m+c+1$ replicas will have at least $m+1$ overlapping nodes
that received a \one message for request $\mu$ from the previous primary.
Thus, there is at least one non-faulty node in that quorum that helps
the protocol to process request $\mu$ in the new view.


\medskip
\noindent
{\bf Step 5:}
Once a replica receives a \three message from the primary 
it checks the view number to be equal to its current view.
Then, the replica inserts the message in its log.
Note that even if the replica has not received a \one message for that request,
as long as the view number is valid and
the message comes from the primary,
the replica considers the request as committed.

If the replica has executed all requests with lower sequence numbers than $n$,
it executes the request.
This ensures that all non-malicious replicas execute requests
in the same order as required to provide the safety property.

\medskip
\noindent
{\bf Step 6:}
When the client receives a \reply message
$\big\langle\text{\REPLY}, \allowbreak \pi, v, ts_{\varsigma}, u  \big\rangle_{\sigma_p}$
with a valid signature
from the primary $p$
and with the same timestamp as the client's request,
it accepts $u$ as the result of the requested operation.

If the client does not receive the reply from the primary after a preset time, the client
may suspect a crashed primary. The client then broadcasts the same request to all replicas.
A replica, upon receiving the client's request, checks if it has already executed the request;
if so, it simply sends the reply message to the client.
The primary will eventually be suspected to be faulty by enough replicas to trigger a view change.

\medskip
\noindent{\bf State Transfer}.
A fault-tolerant protocol must provide a way to checkpoint the state of different replicas.
It is especially required in an asynchronous system where even non-faulty replicas
can fall arbitrarily behind.
It also brings slow replicas up to date
so that they may execute more recent requests.

Similar to \cite{castro1999practical}, in our protocol,
checkpoints are generated periodically when a request
sequence number is divisible by some constant
(checkpoint period).

Trusted primary $p$ produces a checkpoint and multicasts a
$\big\langle\text{\CHECKP}, n,d \big\rangle_{\sigma_p}$ message
to the other replicas, where
$n$ is the sequence number of the
last executed request and $d$ is the digest of the state.
A server considers a checkpoint to be {\em stable} when it
receives a \checkp message for sequence number $n$
signed by trusted primary $p$.
We call this message a {\em checkpoint certificate}, which proves that
the replica's state was correct until that request execution.

Checkpointing not only brings the slow replicas up to date,
but it can also be used as a garbage collection mechanism.
All the messages sent by a replica are kept in a message log in case
they have to be re-sent.
However, when a checkpoint becomes stable,
replicas do not further need to keep messages prior to
the checkpoint in their log and can simply discard
all \one, \two, and \three messages with sequence numbers
less than or equal to the checkpoint's sequence number
from their logs.
They also discard all earlier checkpoints and checkpoint messages.

%\vspace{-1em}
%\medskip
\noindent{\bf View Changes}.
The goal of the view change protocol is to provide liveness by allowing
the system to make progress when a primary fails.
It prevents replicas from waiting indefinitely for requests to execute.
A view change must guarantee that it will not introduce any changes in a
history that has been already completed at a correct client.

Most view change sub-protocols
\cite{el1985availability, el1985efficient, castro1999practical, kotla2007zyzzyva, yin2003separating, castro2003base, cowling2006hq}
require a non-faulty replica to commit a view change message and
when the required number of replicas
suspect that the primary is faulty, the view is changed.
\protocol uses a similar technique in the Lion mode and changes the view
when a trusted primary crashes.
In such a situation, replicas detect the failure and
reach agreement to change the view from $v$ to $v'$.
The primary of new view $v'$ then handles the accepted but not yet committed requests,
and takes care of the new client requests.

View changes are triggered by timeout.
When a replica receives a valid \one message from the primary,
it starts a timer that expires after some defined time $\tau$.
When the backup receives a valid \three message, the timer is stopped,
but if at that point the backup is waiting for a \three message for
some other request, it restarts the timer.
If the timer expires, the backup suspects that the primary is faulty and
starts a view change.

The backup stops accepting \one and \three messages and multicasts a
$\big\langle\text{\VCHANGE}, v+1, n, \xi, \cal P, \cal C \big\rangle$
message to all replicas where
$n$ is the sequence number of the last stable checkpoint known to $r$,
$\xi$ is the checkpoint certificate, and
$\cal P$ and $\cal C$ are two sets of received valid \one 
(without the request message $\mu$)
and \three messages
for requests with a sequence number higher than $n$.

When primary $p'$ of new view $v+1$ receives
$2m+c$ valid \vchange messages
from different replicas, it multicasts a
$\big\langle\text{\NEWV}, v+1, \cal P', \cal C'$$\big\rangle_{\sigma_{p'}}$
message to all replicas where
% $\Sigma$ is the set of $2m+c+1$ valid \vchange messages
% ($2m+c$ messages from other replicas plus its own message), and
$\cal P'$ and $\cal C'$ are two sets of
\one and \three messages respectively
which are constructed as follows.
 
Let $l$ be the sequence number of the latest checkpoint, and
$h$ be the highest sequence number of a \one message in all the received $P$ sets.
For each sequence number $n$ where $l < n \leq h$,
the primary does the following steps:

Step 1: It first checks all \three messages in set $\cal C$ of the received \vchange messages.
If the primary finds a \three message with a valid signature $\sigma_p$
($p$ was the primary of view $v$)
for some request $\mu$
the primary adds a
$\big\langle\big\langle\text{\THREE}, v+1, n  \big\rangle_{\sigma_{p'}}, \mu\big\rangle$
to $\cal C'$

Step 2: If no such \three message is found,
the primary checks the \one messages in $P$ sets:

$\bullet$ If the primary find $2m+c+1$ valid prepare messages for $n$,
it adds a
$\big\langle\big\langle\text{\THREE}, v+1, n, \big\rangle_{\sigma_{p'}}, \mu\big\rangle$
to $\cal C'$.

$\bullet$ Else, if it receives at least one \one message for $n$ that is signed
by the primary of view $v$,
the primary adds a
$\big\langle \big\langle\text{\ONE}, v{+}1, n \big\rangle_{\sigma_{p'}},\mu\big\rangle$
to $\cal P'$.

Step 3: If none of the above situations occur,
there is no valid request for $n$, so
the primary adds a
$\big\langle\text{\ONE}, v{+}1,\allowbreak n, \big\rangle_{\sigma_{p'}},
\mu^{\emptyset}\big\rangle$
to $\cal P'$ where $\mu^{\emptyset}$ is a special no-op command
that is transmitted by the protocol like other requests but leaves the state unchanged.
The third situation happens when no replica has received
a \one message from the previous primary.

Note that, here, in contrast to PBFT, 
since the primary is trusted,
it does not need to put
all the \vchange messages in the \newv message which makes the \newv messages
much smaller.

The primary then inserts all the messages in $\cal P'$ and $\cal C'$
to its log.
It also checks the log to make sure its log contains the latest stable checkpoint.
If not, the primary inserts \checkp messages for the checkpoint $l$ and
discards the earlier information from the log.

Once a replica in view $v$ receives a \newv message from the primary of view $v+1$,
the replica logs all \one and \three messages,
updates its checkpoint in the same way as the primary, and
for each \one message, sends an \two message to the primary.

Note that non-faulty replicas in view $v$ will not accept a \one message for a new view $v' > v$
without having received a \newv message for $v'$.

\medskip
\noindent{\bf Correctness}.
Within a view, since the primary is trusted, safety is ensured as long as the primary does not fail.
If the primary fails a view change is executed.
To ensure safety across the views, as discussed earlier,
the primary waits for $2m+c$ \two messages (considering itself, a quorum of $2m+c+1$)
from different replicas before committing a request $\mu$.
As a result, if the primary fails,
since every two quorums have an intersection
of at least $m+1$ replicas,
there is at least one correct replica in the set of $2m+c+1$ participants of the view change routine
who received \one (and sent \two) messages for
the request $\mu$.
Thus, by the second step of the view change routine, the request will be processed
in the next view.

% The view change protocol ensures liveness by allowing
% the system to make progress when a primary fails.
% The protocol waits for $2m+c+1$ \vchange requests before changing the view.
% Here, to avoid starting the view change too late, we use a similar technique as PBFT \cite{castro1999practical} and
% if a replica receives a set of $m+c+1$ \vchange messages from different replicas,
% it also sends a \vchange message for the smallest view in that set.
% Note that even if all the malicious replicas request a \vchange,
% they cannot force the protocol to change the view.
% In addition, when a replica in view $v$ sends a \vchange message for view $v+1$, it starts a timer $t_{v+1}$.
% If the timer is expired, it sends a \vchange message for view $v+2$ and starts another timer $t_{v+2}$
% where $t_{v+2}$ is larger than $t_{v+1}$ to avoid starting a view change too soon.

\subsection{The Dog Mode: Trusted Primary, Untrusted Backups}\label{sec:mode2}

\begin{algorithm}
\label{algo:dog}
\caption{Steps followed by the primary or a replica in {Dog mode}.}

\begin{algorithmic}[1]
\State \textbf{init():} 
\State    \quad $r$ := $replica\_ id$
\State    \quad $v$ := $view\_ number$ 
\State    \quad if $r = (v \mod S)$, $S$ is private network size:
\State        \qquad $is\_primary$ := \textsf{true}
\State    \quad else if $r = (v \mod P)$ $\in [S,..,S+3m]$, $P$ is public 
\State    \quad network size:
\State        \qquad $is\_proxy$ := \textsf{true\\}

\State \textbf{upon receiving} $\mu = \big\langle\REQ, op, ts_{\varsigma}, \varsigma \big\rangle_{\sigma_{\varsigma}}$ from client $\varsigma$ and \textbf{\textit{is\_primary = true}:}

\State    \quad if \textit{check\_valid\_req($\mu$):}
    
\State    \qquad $n$ := $sequence\_num$
    
\State    \qquad \textbf{send} $\big\langle\big\langle\text{\ONE}, v, n \big\rangle_{\sigma_p}, \mu \big\rangle$ to all {replicas\\}

\State \textbf{upon receiving} $\big\langle\big\langle\text{\ONE}, v, n \big\rangle_{\sigma_p}, \mu \big\rangle$ from primary and \textbf{\textit{is\_proxy = true}}:

\State    \quad if $v$ is valid:
    
\State    \qquad log the message
    
\State    \qquad \textbf{send} $\big\langle\text{\TWO}, v, n, r \big\rangle_{\sigma_r}$ to all {proxies\\}

\State \textbf{upon receiving} $\big\langle\text{\TWO}, v, n, r \big\rangle$ from \textbf{2m+1} proxies:

\State    \quad \textbf{send} $\big\langle\text{\THREE}, v, n, r \big\rangle_{\sigma_{r}}$ to all other proxies
    
\State    \quad \textbf{send} $\big\langle\text{\INFORM}, v, n, r, d \big\rangle_{\sigma_r}$ to all private cloud nodes and non-proxy nodes in public cloud

\State    \quad \textbf{send} $\big\langle\text{\REPLY}, \pi, v, ts_{\varsigma}, u  \big\rangle_{\sigma_r}$ to the client with result $u$

\end{algorithmic}
\end{algorithm}
The Dog mode is proposed to reduce the load on the private cloud.
In the Dog mode of the protocol,
a trusted primary receives a \req message, assigns a sequence number, and
relies on $3m+1$ nodes in the public cloud to process the request.
Since a trusted primary assigns the sequence number to the request before broadcasting,
this reduces the scope of any malicious behaviour.
Note that, in PBFT, when replicas receive a message from the primary,
they perform one round of communication to make sure
all non-faulty replicas agree on a total order for the requests within a view.
However, here, since a trusted primary assigns the sequence numbers, similar to the Lion mode,
there is no need for that round of communication.

We call the $3m+1$ replicas in the public cloud
who receive \req messages from the trusted primary
"proxies".
A replica $i$ in the public cloud is an {\em proxy} in view $v$ if
$i- (v \mod P) \in [S, ...,S+3m]$.
Here since replicas are in the public cloud, $i$ is an integer in $[S, ..., N{-}1]$.
Note that the public cloud might have more than $3m+1$ replicas,
however, $3m+1$ is enough to reach consensus and
any additional replicas may degrade the performance.
In this mode, we also assume that at least one non-faulty replica exists in the private cloud ($S > c$).
The trusted primary of view $v$ is chosen in the same way as the first mode, i.e., $p$ is the primary if
$p = (v \mod S)$.

Similar to the Lion mode,
the normal case operation of the protocol in the Dog mode 
processes a request in six steps.
Figure~\ref{fig:case2} shows the normal case operation of \protocol
with a trusted primary (node $0$).
As before, two replicas are trusted ($S=2$), four replicas are untrusted ($P=4$), $c=1$, and $m=1$.

In the first step, a client sends a \req message $\mu$ to the primary.
In the second step, the primary,
checks the signature and timestamp of the
message $\mu$ to be valid,
assigns a sequence number to the request, and
multicasts a signed \one message
$\big\langle\big\langle\text{\ONE}, v, n \big\rangle_{\sigma_p}, \mu \big\rangle$
to all replicas.

When a proxy receives a \one message from the primary,
it checks the view number to be equal to its view number,
logs the message and sends a signed \two message
$\big\langle\text{\TWO}, v, n, r \big\rangle_{\sigma_r}$
to all the other proxies.
Here, in contrast to the first mode,
the proxy signs its message because it will be used later
in the view change as a proof of receipt of the message.
Note that a malicious proxy might change the sequence number
and multicast it.
Other replicas who receive a \one message from the primary,
only log the message.

When a proxy receives an \two message,
it first validates the signature and the view number, and then
logs the message.
Upon receiving $2m+1$ matching \two messages
(including its own message),
a proxy $r$ multicasts a \three message
$\big\langle\text{\THREE}, v, n, r \big\rangle_{\sigma_{r}}$
to the other proxies.
Each proxy $r$ also sends a signed \inform message
$\big\langle\text{\INFORM}, v, n, r, d \big\rangle_{\sigma_r}$
to all the nodes in the private cloud and all non-proxy nodes in the public cloud.
The {\em \inform} message contains view number $v$, sequence number $n$,
identifier $r$, and message digest $d$ (to validate the message)
to inform them that such a request is committed.
Non-proxy nodes wait for $2m+1$ valid matching \inform messages from different proxies
which are also matched by the \one message that they received from the primary
before executing the request.

% Note that if a proxy $i$ receives $2m+1$
% matching \two messages
% for request $\mu$ in view $v$ with sequence number $n$,
% then, it is not possible for any replica $j$ (including $i=j$) to receive $2m+1$ matching \two messages
% for another request $\mu'$ in view $v$ with sequence number $n$.
% In fact, since a trusted primary assigns sequence numbers and
% the total number of executers is $3m+1$,
% these two quorums of size $2m+1$ have an intersection of at least $m+1$ replicas
% which means at least $1$ non-malicious replica sends two \two messages with the same view and sequence number.
% But this is not possible because the replica is non-malicious.

If the proxy has executed all requests with sequence numbers lower than $n$, it also executes the request $n$
and sends a \reply message
$\big\langle\text{\REPLY}, \pi, v, ts_{\varsigma}, u  \big\rangle_{\sigma_r}$ to the client where $u$ is the result
of the requested operation.

Any other replica that receives $2m+1$ matching \three messages
from the proxies with
valid signatures,
correct message digest, and
view numbers equal to its view number
considers the request as committed, and executes the request.
Note that since all the replicas receive \one messages from the primary,
they have access to the request and can execute it.
The client also waits for $2m+1$ matching \reply messages
from the proxies
with a valid signature and the same timestamp
as its request timestamp to accept the result.

The client multicasts the request to the proxies if it has not received
a valid reply. The proxies re-send the result if the request has already
been processed. Otherwise, similar to the first mode,
eventually the primary will be suspected to be faulty by enough replicas and a view change will be triggered.

As can be seen in Figure~\ref{fig:case2}
Since a trusted primary assigns sequence numbers, the protocol, similar to Paxos, needs two phases to process requests.
However, since the protocol tolerates malicious failures, the number of messages in terms of the number of replicas,
similar to PBFT, is quadratic.
Here, there are totally $N+(3m+1)^2+ (3m+1)*N$ messages exchanged where $3m+1$ is the total number of proxies.
In this particular example, since $m=1$, all replicas in the public cloud are proxies.



\medskip
\noindent{\bf State Transfer}.
Checkpointing in the Dog mode works in the same way as
the Lion mode.
Trusted primary $P$ multicasts a signed \checkp message
to all other replicas with the sequence number of the
last executed request and the digest of the state.
Upon receiving a \checkp message from the primary,
a server considers that a checkpoint is {\em stable} and logs
the message which is used later as a
{\em checkpoint certificate}.

\medskip
\noindent{\bf View Changes}.
In the Dog mode of the protocol, view change happens when the trusted primary is suspected to have crashed.
Here, similar to the Lion mode, we rely on the primary of new view to
handle the prepared but not yet committed requests.
However, since the nodes in the public clouds are processing
the requests, they are the ones who send \vchange messages.
A proxy,
%i.e., one of the $3m+1$ replica in the public cloud,
%whose timer is expired
multicasts a \vchange message
$\big\langle\text{\VCHANGE}, v+1, n, \xi, \cal P \big\rangle$
to all the nodes in the public cloud and the primary of the next view where
$\xi$ is the checkpoint certificate for sequence number $n$,
and
$\cal P$ is
the set of received valid \one messages
with a sequence number higher than $n$.

Primary $p'$ of the new view waits for $2m+1$ valid \vchange messages
from the public cloud and multicast a \newv message
$\big\langle\text{\NEWV}, v+1, \cal P'$ $\big\rangle_{\sigma_{p'}}$
to all the replicas where
for each sequence number $n$
(between the latest checkpoint and the highest sequence number of a \one message),
if there is any valid \one message in set $\cal P$
of the received \vchange messages,
the primary adds a
$\big\langle\text{\ONE}, v+1, n  \big\rangle_{\sigma_{p'}}$
to $\cal P'$.
Else, there is no valid request for $n$, so
similar to the Lion mode, 
the primary adds a no-op \one message to $\cal P'$.

Here, again, since the primary is trusted it does not need
to include \vchange messages in the \newv message.
The primary then inserts all the messages in $\cal P'$
to its log and updates its checkpoint, if needed.

Once a proxy of view $v+1$ receives a \newv message from the primary of view $v+1$,
the proxy logs all \one messages,
updates its checkpoint, and
multicasts an \two message to all the proxies
for each \one message in $\cal P'$.
Other replicas also receive the \newv message to inform them that the view is changed.

\medskip
\noindent{\bf Correctness}.
Since the primary is trusted, safety in the Dog mode is satisfied
similar to the Lion mode except that since
the protocol has $3m+1$ participants, to commit a message $2m+1$ \two messages are needed.
%Similarly, to ensure liveness, the view change routine waits for $2m+1$ \vchange messages to trigger.


\subsection{Peacock Mode: Untrusted Primary, Untrusted Backups}\label{sec:mode3}

The third mode of the protocol, the Peacock mode, is presented to handle two different situations.
First, when there is a large network distance between the private
and the public cloud and
the latency due to one more phase is less than the latency of
exchanging messages between the two clouds.
Second, when the private cloud is heavily loaded and the public cloud can
handle the requests by itself for load balancing.
In both situations, the nodes in the private cloud become passive replicas in the agreement routine
and are only informed about the committed messages.
However, they still may participate in the view change routine.

In peacock mode, \protocol completely relies on $3m+1$ nodes in the public cloud to
process the requests using PBFT \cite{castro1999practical}.
The untrusted primary of view $v$ in the Peacock mode
is a replica $p$ such that $p = (v \mod P) + S$.
Similar to the Dog mode, since there might be more than $3m+1$ replicas in the public cloud,
in each view, we choose $3m+1$ of them as the proxies.
Node $i$ is a proxy of view $v$ if $i- (v \mod P) \in [S, ...,S+3m]$.
This ensures that the primary is always a proxy.
As can be seen in Figure~\ref{fig:case3}, the total number of exchanged messages
in the Peacock mode is $N+ 2 * (3m+1)^2 + (1+S) * (3m+1)$.

% The normal case operation of this mode is similar to PBFT \cite{castro1999practical}
% in terms of the required number of phases (three) and the message passing pattern.
% Figure~\ref{fig:case3} show the normal case operation of \protocol
% in the Peacock mode.
% As can be seen, the replicas in the private cloud have no participation
% in any phases and are only informed about the committed request.

% In particular, the algorithm works as follow.
% A client sends a request $\mu$ to an untrusted primary.
% The primary then, validates the message,
% assigns a sequence number to the request
% and multicasts a signed {\em \zero} message along with the request to all the replicas.
% The primary also, adds the digest of $\mu$ to the message which is used later
% by the other replicas to validate the message.

% Upon receiving a valid \zero message from the primary,
% a proxy checks the message and multicasts
% a signed \one message to all other proxies.
% Nodes other than proxies only log the received \zero message.
% When a proxy receives $2m+1$ valid matching \one messages from other proxies for a request,
% it multicasts a \three message to all other proxies.
% As soon as a proxy has accepted $2m+1$ commits (possibly including its own)
% from different proxies that match the \zero message for the request,
% it executes the request and sends
% a reply including the result of the execution to the client.
% The client waits for $m+1$ valid replies from different proxies of that view
% before accepting the result.
% When the request is committed, each proxy $r$ also sends a signed \inform message
% $\big\langle\text{\INFORM}, v, n, r, d \big\rangle_{\sigma_r}$
% to all the nodes in the private cloud and all non-proxy nodes in the public cloud.
% Other nodes also wait for $m+1$ valid matching \inform messages
% from different proxies before executing the request.


% \medskip
% \noindent{\bf State Transfer}.
% In the Peacock mode of the protocol, since the primary might be
% a malicious node, we can not rely on it to produce the checkpoint, so
% all the replicas participate in checkpointing.
% Once a replica $r$ executes a request with a sequence number $n$ equal to
% the checkpoint period,
% it produces a \checkp message
% $\big\langle\text{\CHECKP}, n,d,r \big\rangle_{\sigma_r}$
% and multicasts the message to the other replicas.
% The replica has to sign the \checkp message because it will be used later
% in view changes.
% A server considers that a checkpoint is {\em stable} when it
% receives $2m+c+1$ \checkp messages for sequence number $n$ with the same digest $d$
% from different replicas (possibly including its own message).
% This set of messages is called a {\em checkpoint certificate}, which
% proves that the replica's state was correct until that request execution.

\medskip
\noindent{\bf View Changes}.
In the Peacock mode, We rely on a trusted node in the private cloud, called {\em transferer}, to change the view.
Indeed, instead of the primary of the new view, a transferer changes the view.
Replica $t$ in the private cloud is the transferer of view $v'$
(changes the view from $v$ to $v'$)
if $t = (v'\mod S$).
Choosing a transferer to change views helps in
minimizing the size of \newv messages and
more importantly, reduce the delay between the request and its reply.
Because even if there are consecutive malicious primary nodes,
since the transferer takes care of the uncommitted requests of view $v$,
the protocol does not carry the messages from one view to another.
In contrast, in PBFT, it is possible that a valid request in view $v$
be committed in view $v+m$ (when there are $m$ consecutive primaries).
Other than the transferer, view change in the Peacock mode is similar to PBFT.
% proxies multicast \vchange messages consisting of
% the sequence number $n$ of the last stable checkpoint
% known to the proxy,
% the checkpoint certificate $\xi$ (a set of $2m+c+1$ \checkp messages), and
% a set $\cal A$ consisting of $2m+1$ valid \two messages
% for each request with a sequence number higher than $n$.
% When the transferer $t$ of new view $v+1$ receives
% $2m+1$ valid \vchange messages
% from different proxies of view $v$,
% it multicasts a \newv message to all replicas in both public and private clouds.
% The \newv message contains
% a set of \one messages $\cal P'$ where
% for each sequence number $n$,
% if the transferer finds a set of $2m+1$ valid \two message
% in set $\cal A$ of a received \vchange messages,
% it adds a \one message 
% $\big\langle\text{\ONE}, v{+}1, n, d \big\rangle_{\sigma_{p'}}$
% to $\cal P'$.
% Else, the transferer adds a no-op \one message
% $\big\langle\text{\ONE}, v{+}1, n, d^{\emptyset} \big\rangle_{\sigma_{p'}}$
% to $\cal P'$.
% Here, since the transferer is trusted, it does not need to put
% all the \vchange messages in the \newv message.

% The transferer then logs all the \one messages that are sent
% and updates its checkpoint if needed.
% proxies, on the other hand, log all the \one messages,
% update their checkpoints, and send an \two message to all other proxies
% for each \one message.
% Other nodes in the private and public cloud receive the \newv to be informed that
% the view is changed.
Once the transferer has changed the view and the new primary receives the \newv message from the transferer,
it starts to process new requests in view $v+1$.

% In this mode, we might have consecutive views with malicious primaries.
% As a result, the uncommitted requests in view $v$ will be carried from one view to another.
% However, since there are at most $m$ malicious replicas,
% in the worst case scenario, after $m$ view changes, a non-faulty replica becomes the primary.

\medskip
\noindent{\bf Correctness}. In the Peacock mode, the protocol ensures safety and liveness similar to PBFT \cite{castro1999practical}.

\subsection{Dynamic Mode Switching}\label{sec:switch}

We presented three different modes of \protocol and
explained when each mode is useful.
Now, we show how to dynamically switch between different modes.

An enterprise might prefer to use the Lion mode of \protocol,
because it needs fewer phases
(in comparison to the Peacock mode) and
less number of message exchanges
(in comparison to the Dog or Peacock mode).
However, if the private cloud becomes heavily loaded, or
at some point, a high percentage of requests are sent by clients
that are far from the private cloud and much closer to the public cloud,
it might be beneficial to switch to the Dog or Peacock mode.
\protocol might also plan to switch back to the Lion mode,
e.g., when the load on the private cloud is reduced.
To change the mode, the protocol also has to change the view, because the primary
and the set of participant replicas might be different in different modes.
Therefore, to handle a mode change, the protocol, first performs a
view change, and then the primary of the new view in the new mode
starts to process the new requests.

For the switch to happen
a {\em trusted} replica $s$ multicasts a
$\big\langle\text{\MCHANGE}, v+1, \pi' \big\rangle_{\sigma_s}$ to
all the replicas where $\pi'$ is the new mode of the protocol,
i.e., Lion, Dog, or Peacock.
When the protocol wants to switch to the Lion or Dog mode, replica $s$ is the primary of view $v+1$, and
when it switches to the Peacock mode, replica $s$ is the transferer of view $v+1$.

\subsection{Discussion}\label{sec:disc}

{\footnotesize
\begin{table}[t]\label{tbl:comp}
\caption{Comparison of Fault-tolerant protocols}
\begin{center}
\setlength\tabcolsep{1.5pt}
\begin{tabular}{ |c|c|c|c|c|c| } 
%  \hline
%  & Lion & Dog & Peacock & Paxos & PBFT & UpRight  \\ 
%  \hline
% \# of phases & $2$ & $2$ & $3$ & $2$ & $3$ & $2$\\ 
%  \hline
% \# of messages & $\calo(n)$ & $\calo(n^2)$ & $\calo(n^2)$ & $\calo(n)$ & $\calo(n^2)$ & $\calo(n^2)$\\
%  \hline
% Receiving Network & $3m{+}2c{+}1$ & $3m{+}1$ & $3m{+}1$ & $2f{+}1$ & $3f{+}1$ & $3m{+}2c{+}1$\\ 
%   \hline
% Quorum size & $2m{+}c{+}1$ & $2m{+}1$ & $2m{+}1$ & $f{+}1$ & $2f{+}1$ & $2m{+}c{+}1$\\ 
  \hline
  Protocol & \# of phases & \# of messages & Receiving Network & Quorum size\\
 \hline
  Lion & $2$ & $\calo(n)$ & $3m{+}2c{+}1$ & $2m{+}c{+}1$\\
 \hline
  Dog & $2$ & $\calo(n^2)$ & $3m{+}1$ & $2m{+}1$\\
 \hline
  Peacock & $3$ & $\calo(n^2)$ & $3m{+}1$ & $2m{+}1$\\
 \hline
  Paxos & $2$ & $\calo(n)$ & $2f{+}1$ & $f{+}1$\\
 \hline
  PBFT & $3$ & $\calo(n^2)$ & $3f{+}1$ & $2f{+}1$\\
 \hline
  UpRight & $2$ & $\calo(n^2)$ & $3m{+}2c{+}1$ & $2m{+}c{+}1$\\
 \hline
\end{tabular}
\end{center}
\end{table}
}
In this section, we compare different modes of \protocol with three well-known protocols:
the crash fault-tolerant protocol Paxos \cite{lamport2001paxos},
the Byzantine fault-tolerant protocol PBFT \cite{castro1999practical}, and
the hybrid fault-tolerant protocol UpRight \cite{clement2009upright}.
We consider four parameters in this camparison:
1) the number of communication phases,
2) the number of message exchanges,
3) the receiving network size, and
4) the quorum size.
The results are reported in Table~\ref{tbl:comp}.

Being aware of where a crash or a malicious failure may occur and as a result
choose a trusted primary
simply reduces one phase of communication.
In fact, in PBFT,
the {\tt prepare} phase is needed only to make sure that non-faulty replicas receive matching 
{\tt pre-prepare} messages from the primary.
In contrast, in the Lion and Dog modes of \protocol,
since the primary is a trusted node, replicas receive the same message
from the primary, thus there is no need for that phase of communication and
the requests, similar to Paxos , are processed in two phases
( while in contrast to Paxos malicious failures can occur).
In comparison to Upright,
although Upright processes the requests in two phases,
it utilizes the speculative execution technique introduced by Zyzzyva \cite{kotla2007zyzzyva}
which becomes very costly (i.e., needs 4 rounds of communications) in the presence of failures.
Note that the speculative execution technique can easily be applied to \protocol as well.

The number of message exchanges in the Lion mode is similar to Paxos and is linear
in terms of the total number of replicas.
In the Dog mode, the number of messages is quadratic,
however it is still much less than PBFT
(since it has one phase of $n$-to-$n$ communication instead of two).
Upright also has a quadratic number of messages.

The the Lion mode, similar to Upright, needs $3m+2c+1$ nodes receive a client request.
In the Dog mode, however, only the trusted primary and $3m+1$ nodes from the public cloud participate in each phase.
Since the Peacock mode utilizes PBFT, the number of phases and message exchanges are the same as PBFT.
However, since the primary is in the public cloud, communicating with the private cloud has no advantage,
thus it proceeds with $3m+1$ nodes instead of $3m+2c+1$ as in the Lion mode and UpRight.


